A Neural Network Alternative to Tree-based Models

Tabular datasets are widely used in scientific disciplines such as biology. While these disciplines have already adopted AI methods to enhance their findings and analysis, they mainly use tree-based methods due to their interpretability. At the same time, artificial neural networks have been shown to offer superior flexibility and depth for rich and complex non-tabular problems, but they are falling behind tree-based models for tabular data in terms of performance and interpretability. Although sparsity has been shown to improve the interpretability and performance of ANN models for complex non-tabular datasets, enforcing sparsity structurally and formatively for tabular data before training the model, remains an open question. To address this question, we establish a method that infuses sparsity in neural networks by utilising attention mechanisms to capture the features' importance in tabular datasets. We show that our models, Sparse TABular NET or sTAB-Net with attention mechanisms, are more effective than tree-based models, reaching the state-of-the-art on biological datasets. They further permit the extraction of insights from these datasets and achieve better performance than post-hoc methods like SHAP.

==> sn-jnl__latexbib.tex <==
% %%
% %% This is file `sn-jnl.cls',
% %% generated with the docstrip utility.
% %%
% %% The original source files were:
% %%
% %% classes.dtx  (with options: `sn-jnl')
% %%
% %% This is a generated file.
% %%
% %% Copyright 1993 1994 1995 1996 1997 1998 1999 2000 2001 2002 2003 2004 2005 2006 2007 2008 2009
% %% The LaTeX3 Project and any individual authors listed elsewhere
% %% in this file.
% %%
% %% This file was generated from file(s) of the LaTeX base system.
% %% --------------------------------------------------------------
% %%
% %% It may be distributed and/or modified under the
% %% conditions of the LaTeX Project Public License, either version 1.3c
% %% of this license or (at your option) any later version.
% %% The latest version of this license is in
% %%    http://www.latex-project.org/lppl.txt
% %% and version 1.3c or later is part of all distributions of LaTeX
% %% version 2005/12/01 or later.
% %%
% %% This file has the LPPL maintenance status "maintained".
% %%
% %% This file may only be distributed together with a copy of the LaTeX
% %% base system. You may however distribute the LaTeX base system without
% %% such generated files.
% %%
% %% The list of all files belonging to the LaTeX base distribution is
% %% given in the file `manifest.txt'. See also `legal.txt' for additional
% %% information.
% %%
% %% The list of derived (unpacked) files belonging to the distribution
% %% and covered by LPPL is defined by the unpacking scripts (with
% %% extension .ins) which are part of the distribution.
% %% \CharacterTable
% %%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
% %%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
% %%   Digits        \0\1\2\3\4\5\6\7\8\9
% %%   Exclamation   \!     Double quote  \"     Hash (number) \#
% %%   Dollar        \$     Percent       \%     Ampersand     \&
% %%   Acute accent  \'     Left paren    \(     Right paren   \)
% %%   Asterisk      \*     Plus          \+     Comma         \,
% %%   Minus         \-     Point         \.     Solidus       \/
% %%   Colon         \:     Semicolon     \;     Less than     \<
% %%   Equals        \=     Greater than  \>     Question mark \?
% %%   Commercial at \@     Left bracket  \[     Backslash     \\
% %%   Right bracket \]     Circumflex    \^     Underscore    \_
% %%   Grave accent  \`     Left brace    \{     Vertical bar  \|
% %%   Right brace   \}     Tilde         \~}
% \NeedsTeXFormat{LaTeX2e}[1995/12/01]
% \ProvidesClass{sn-jnl}
%               [2019/11/18 v0.1: An authoring template for Springer Journal articles]

% \newif\if@restonecol
% \newif\if@titlepage   \@titlepagefalse
% \newif\if@cropmarkson \@cropmarksonfalse
% \newif\ifDoublecol    \Doublecolfalse%
% \newif\ifpagebody\global\pagebodyfalse%
% \newif\if@iicol\global\@iicolfalse%
% \newif\if@bibcomment\global\@bibcommentfalse%
% \newif\if@referee\global\@refereefalse%
% \newif\if@vrulerlinenumberon\global\@vrulerlinenumberonfalse%
% \newif\if@pdflatex\global\@pdflatexfalse%
% \newif\if@remarkboxon\global\@remarkboxonfalse%

% \newif\if@Numbered@refstyle\global\@Numbered@refstylefalse% Namedate
% \newif\if@Spr@basic@refstyle\global\@Spr@basic@refstylefalse% 1.Basic Springer Nature Reference Style/Chemistry Reference Style -> sn-basic.bst
% \newif\if@Mathphys@numrefstyle\global\@Mathphys@numrefstylefalse% 2.Math and Physical Sciences Reference Style -> sn-mathphys.bst
% \newif\if@Mathphys@ayrefstyle\global\@Mathphys@ayrefstylefalse% 2.Math and Physical Sciences Reference Style -> sn-mathphys.bst
% \newif\if@APS@refstyle\global\@APS@refstylefalse% 3.American Physical Society (APS) Reference Style -> sn-APS.bst
% \newif\if@Vancouver@numrefstyle\global\@Vancouver@numrefstylefalse% 4.Vancouver Reference Style -> sn-vancouver.bst
% \newif\if@Vancouver@ayrefstyle\global\@Vancouver@ayrefstylefalse% 4.Vancouver Reference Style -> sn-vancouver.bst
% \newif\if@APA@refstyle\global\@APA@refstylefalse% 5.APA-based Social Sciences/Psychology Reference Style -> sn-apacite.bst
% \newif\if@Chicago@refstyle\global\@Chicago@refstylefalse% 6.Chicago-based Humanities Reference Style -> sn-chicago.bst
% \newif\if@Standard@Nature@refstyle\global\@Standard@Nature@refstylefalse% 7.Standard Nature Research Style -> sn-nature.bst

% %% Template Options
% \DeclareOption{a4paper}{\PassOptionsToPackage{a4}{crop}}
% \DeclareOption{a3paper}{\PassOptionsToClass{a3paper}{article}\PassOptionsToPackage{a3}{crop}}
% \DeclareOption{centre}{\PassOptionsToPackage{center}{crop}}
% \DeclareOption{crop}{\PassOptionsToPackage{frame}{crop}\global\@cropmarksontrue}
% \DeclareOption{nocrop}{\PassOptionsToPackage{off}{crop}\global\@cropmarksontrue}
% \DeclareOption{info}{\PassOptionsToPackage{info}{crop}}
% \DeclareOption{noinfo}{\PassOptionsToPackage{noinfo}{crop}}

% %% Classfile Options
% \DeclareOption{oneside}{\@twosidefalse \@mparswitchfalse}
% \DeclareOption{twoside}{\@twosidetrue  \@mparswitchtrue}
% \DeclareOption{draft}{\setlength\overfullrule{5pt}}
% \DeclareOption{titlepage}{\@titlepagetrue}
% \DeclareOption{notitlepage}{\@titlepagefalse}
% \DeclareOption{onecolumn}{\@twocolumnfalse}
% \DeclareOption{twocolumn}{\@twocolumntrue}
% \DeclareOption{openbib}{\let\if@openbib\iftrue}
% \DeclareOption{pagegrid}{\global\pagebodytrue}%
% \DeclareOption{iicol}{\global\@iicoltrue}%
% \DeclareOption{bibcomment}{\global\@bibcommenttrue}%
% \DeclareOption{referee}{\global\@refereetrue}%
% \DeclareOption{lineno}{\global\@vrulerlinenumberontrue}%
% \DeclareOption{pdflatex}{\global\@pdflatextrue}%
% \DeclareOption{remarkboxoff}{\global\@remarkboxonfalse}%

% \DeclareOption{sn-basic}{\global\@Spr@basic@refstyletrue}%
% \DeclareOption{sn-mathphys-num}{\global\@Mathphys@numrefstyletrue}%
% \DeclareOption{sn-mathphys-ay}{\global\@Mathphys@ayrefstyletrue}%
% \DeclareOption{sn-aps}{\global\@APS@refstyletrue}%
% \DeclareOption{sn-vancouver-num}{\global\@Vancouver@numrefstyletrue}%
% \DeclareOption{sn-vancouver-ay}{\global\@Vancouver@ayrefstyletrue}%
% \DeclareOption{sn-apa}{\global\@APA@refstyletrue}%
% \DeclareOption{sn-chicago}{\global\@Chicago@refstyletrue}%
% \DeclareOption{sn-nature}{\global\@Standard@Nature@refstyletrue}%

% \DeclareOption{Numbered}{\global\@Numbered@refstyletrue}%
% %\DeclareOption{NameDate}{\global\@Numbered@refstylefalse}%


% %%\ExecuteOptions{twosidecrop,crop,centre,info,croppage}
% \ProcessOptions
% \LoadClass[twoside,fleqn]{article}

% \gdef\refereedefns{%
% \if@referee%
% \usepackage{setspace}%
% \doublespacing%
% \fi}%
% \refereedefns%

% %% General Packages Used
% %
% %\AtBeginDocument{%
% %%\newcommand*\ExtraParaSkip{12pt}%
% %\SetFootnoteHook{\hspace*{-8pt}}%
% %\DeclareNewFootnote{A}[gobble]%
% %\setlength{\skip\footinsA}{0pt}
% %}%
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%% Fonts & Sizes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% %% Fonts Used
% %%\RequirePackage[T1]{fontenc}%
% %
% \DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}%
% \DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}%
% \DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}%
% \DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}%
% \DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}%
% \DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}%
% \DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}%
% \DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}%
% \DeclareRobustCommand*\mit{\@fontswitch\relax\mathnormal}%
% %
% \renewcommand\normalsize{%
%    \@setfontsize\normalsize{10bp}{12bp}%
%    \abovedisplayskip 12\p@ \@plus2\p@ \@minus1\p@
%    \abovedisplayshortskip \z@ \@plus3\p@%
%    \belowdisplayshortskip 3\p@ \@plus3\p@ \@minus3\p@%
%    \belowdisplayskip \abovedisplayskip%
%    \let\@listi\@listI}%
% \normalsize%
% %
% \newcommand\medsize{%
%    \@setfontsize\small\@xipt{13}%
%    \abovedisplayskip 5\p@ \@plus3\p@ \@minus4\p@
%    \abovedisplayshortskip \z@ \@plus2\p@
%    \belowdisplayshortskip 3\p@ \@plus2\p@ \@minus2\p@
%    \def\@listi{\leftmargin\leftmargini
%                \topsep 4\p@ \@plus2\p@ \@minus2\p@
%                \parsep 2\p@ \@plus\p@ \@minus\p@
%                \itemsep \parsep}%
%    \belowdisplayskip \abovedisplayskip}%
% %
% \renewcommand\small{%
%    \@setfontsize\small\@ixpt{11}%
%    \abovedisplayskip 5\p@ \@plus3\p@ \@minus4\p@
%    \abovedisplayshortskip \z@ \@plus2\p@
%    \belowdisplayshortskip 3\p@ \@plus2\p@ \@minus2\p@
%    \def\@listi{\leftmargin\leftmargini
%                \topsep 4\p@ \@plus2\p@ \@minus2\p@
%                \parsep 2\p@ \@plus\p@ \@minus\p@
%                \itemsep \parsep}%
%    \belowdisplayskip \abovedisplayskip}%
% %
% \renewcommand\footnotesize{%
%    \@setfontsize\footnotesize{7}{8}%
%    \abovedisplayskip 5\p@ \@plus2\p@ \@minus4\p@
%    \abovedisplayshortskip \z@ \@plus\p@
%    \belowdisplayshortskip 3\p@ \@plus\p@ \@minus2\p@
%    \def\@listi{\leftmargin\leftmargini
%                \topsep 3\p@ \@plus\p@ \@minus\p@
%                \parsep 2\p@ \@plus\p@ \@minus\p@
%                \itemsep \parsep}%
%    \belowdisplayskip \abovedisplayskip}
% %
% \renewcommand\scriptsize{\@setfontsize\scriptsize\@ixpt\@ixpt}%
% \newcommand\scrisize{\@setfontsize\scrisize{9.3}{9}}%
% \renewcommand\tiny{\@setfontsize\tiny\@vpt\@vipt}%
% \renewcommand\large{\@setfontsize\large{12}{14}}%
% \newcommand\larg{\@setfontsize\larg{11}{13}}%
% \renewcommand\Large{\@setfontsize\Large{16}{18}}%
% \renewcommand\LARGE{\@setfontsize\LARGE\@xviipt{22}}%
% \renewcommand\huge{\@setfontsize\huge\@xxpt{25}}%
% \renewcommand\Huge{\@setfontsize\Huge\@xxvpt{30}}%
% %
% \DeclareMathSizes{\@ixpt}{\@ixpt}{7}{5}%
% \DeclareMathSizes{\@xpt}{\@xpt}{7}{5}%
% \DeclareMathSizes{\@xipt}{\@xipt}{7}{5}%
% %
% \DeclareRobustCommand*\textsubscript[1]{%
%   \@textsubscript{\selectfont#1}}%
% %
% \def\@textsubscript#1{%
%   {\m@th\ensuremath{_{\mbox{\fontsize\sf@size\z@#1}}}}}%
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%% Layout Settings %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% %%\RequirePackage{geometry}%
% %
% \newlength\columnhsize%
% %
% %% Regular Pages (for Opening page - redefined)
% %
% \if@iicol%
% %
% %% for double column used sn-medium design trim and page size %%
% %
% \setlength\headheight{12pt}%
% \setlength\headsep{5.15mm}%
% %
% \setlength\columnsep{8mm}%
% \setlength\columnhsize{76mm}%
% %
% \setlength\maxdepth{0pt}%
% \setlength\footnotesep{7\p@}%
% \setlength{\skip\footins}{18\p@ \@plus 6\p@ \@minus 3\p@}%
% %
% \RequirePackage[%
%     reversemp,
%     paperwidth=210mm,
%     paperheight=297mm,
%     top={26mm},
%     headheight={12pt},
%     headsep={5.15mm},
%     text={160mm,216mm},
%     marginparsep=5mm,
%     marginparwidth=12mm,
%     bindingoffset=6mm,
%     footskip=10.13mm,twocolumn]{geometry}%
% %
% \renewcommand\footnoterule{%
%   \kern3\p@%
%   \hrule \@height.2mm \@width\columnwidth%
%   \kern5.5\p@}%
% %
% \else%
% %% For single column used smallcond design trim and page size %%
% \RequirePackage[%
%     reversemp,
%     paperwidth=210mm,
%     paperheight=297mm,
%     top={26mm},
%     headheight={5.5pt},
%     headsep={5.6mm},
%     text={31pc,194.25mm},
%     marginparsep=5mm,
%     marginparwidth=12mm,
%     bindingoffset=6mm,
%     footskip=10mm]{geometry}
% %
%     \setlength\maxdepth{0pt}%
%     \setlength\columnsep{5mm}%
%     \setlength{\marginparsep}{5mm}%
%     \setlength{\marginparwidth}{12mm}%
%     \setlength\footnotesep{5.75\p@}%
%     \setlength{\skip\footins}{8\p@ \@plus 4\p@ \@minus 0\p@}%
% %
% \renewcommand\footnoterule{%
%   \kern3\p@%
%   \ifodd\c@page%
%      \hrule \@height.2mm \@width\textwidth%
%   \else%
%      \hrule \@height.2mm \@width37mm
%   \fi%
%   \kern5.5\p@}%
% %
% \fi%
% %
% %
% \setlength\parindent{1.5em}%
% %
% \def\StepUpCounter#1{\global\advance#1by 1\relax}%
% \def\StepDownCounter#1{\global\advance#1by -1\relax}%
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%% Pagination Settings %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % Line spacing
% \setlength\lineskip{1\p@}%
% \setlength\normallineskip{1\p@}%
% %%\renewcommand\baselinestretch{1.5}%
% \parskip=0pt%
% %
% % Page break penalties
% %
% \@lowpenalty   51
% \@medpenalty  151
% \@highpenalty 301
% %
% % Disallow widows and orphans
% %
% \clubpenalty 10000
% \widowpenalty 10000
% %
% % Disable page breaks before equations, allow pagebreaks after
% % equations and discourage widow lines before equations.
% %
% \displaywidowpenalty 100
% \predisplaypenalty   10000
% \postdisplaypenalty  0
% %
% % Set these global demerits
% %
% \doublehyphendemerits 1000000   % corresponds to badness 800
% \finalhyphendemerits  1000000  % corresponds to badness 1000
% %
% % Allow loose lines rather than overfull lines
% %
% \vbadness=9999
% \tolerance=9999
% %
% % Allow breaking the page in the middle of a paragraph
% %
% \interlinepenalty 0
% %
% % Disallow breaking the page after a hyphenated line
% \brokenpenalty 10000
% %
% % Hyphenation; don't split words into less than three characters
% \lefthyphenmin=3
% \righthyphenmin=3
% %
% % Float placement parameters
% %
% % The total number of floats that can be allowed on a page.
% \setcounter{totalnumber}{3}
% %
% % The maximum number of floats at the top and bottom of a page.
% \setcounter{topnumber}{5}
% \setcounter{bottomnumber}{5}
% %
% % The maximum part of the top or bottom of a text page that can be
% % occupied by floats. This is set so that at least four lines of text
% % fit on the page.
% \renewcommand\topfraction{.921}
% \renewcommand\bottomfraction{.921}

% % The minimum amount of a text page that must be occupied by text.
% % This should accomodate four lines of text.
% \renewcommand\textfraction{.13}

% % The minimum amount of a float page that must be occupied by floats.
% \renewcommand\floatpagefraction{.887}

% % The same parameters repeated for double column output
% \renewcommand\dbltopfraction{.88}
% \renewcommand\dblfloatpagefraction{.88}

% % Space between floats
% \setlength\floatsep{18\p@ \@plus 4\p@ \@minus 2\p@}

% % Space between floats and text
% \setlength\textfloatsep{15\p@ \@plus 4\p@ \@minus 2\p@}

% % Space above and below an inline figure
% \setlength\intextsep   {18\p@ \@plus 4\p@ \@minus 2\p@}

% % For double column floats
% \setlength\dblfloatsep    {20\p@ \@plus 4\p@ \@minus 2\p@}
% \setlength\dbltextfloatsep{15\p@ \@plus 4\p@ \@minus 2\p@}

% \hyphenation{Figure Figures Table Tables Equation Equations Section Sections Appendix Theorem Lemma}


% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%% Math Settings %%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%% For above/below spacing  
% \def\eqnarray{%
%    \stepcounter{equation}%
%    \def\@currentlabel{\p@equation\theequation}%
%    \global\@eqnswtrue
%    \m@th
%    \global\@eqcnt\z@
%    \tabskip\@centering
%    \let\\\@eqncr
%    $$\everycr{}\halign to\displaywidth\bgroup
%        \hskip\@centering$\displaystyle\tabskip\z@skip{##}$\@eqnsel
%       &\global\@eqcnt\@ne\hskip \tw@\arraycolsep \hfil${##}$\hfil
%       &\global\@eqcnt\tw@ \hskip \tw@\arraycolsep
%          $\displaystyle{##}$\hfil\tabskip\@centering
%       &\global\@eqcnt\thr@@ \hb@xt@\z@\bgroup\hss##\egroup
%          \tabskip\z@skip
%       \cr
% }
% \def\endeqnarray{%
%       \@@eqncr
%       \egroup
%       \global\advance\c@equation\m@ne
%    $$\@ignoretrue
% }
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%% Titles %%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% \renewcommand\refname{References}%
% \renewcommand\figurename{Fig.}% defined as per springer style 
% \renewcommand\tablename{Table}%
% \renewcommand\appendixname{Appendix}%
% \renewcommand\abstractname{Abstract}%
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%% Article Front Matter %%%%%%%%%%%%%%%%%%%%%%%%%%%
% %

% \def\raggedleft{\leftskip0pt plus 1fil\parfillskip=0pt\relax}%
% \def\raggedright{\rightskip0pt plus 1fil\parfillskip=0pt\relax}%
% \def\raggedcenter{\leftskip=0pt plus 0.5fil\rightskip=0pt plus 0.5fil%
% \parfillskip=0pt\let\hb=\break}%
% \def\titraggedcenter{\leftskip=12pt plus 0.5fil\rightskip=12pt plus 0.5fil%
% \parfillskip=0pt\let\hb=\break}%
% \def\absraggedcenter{\leftskip=24pt plus 0.5fil\rightskip=24pt plus 0.5fil%
% \parfillskip=0pt\let\hb=\break}%

% %
% %%% Font Def
% \def\Artcatfont{\reset@font\fontsize{8bp}{10bp}\selectfont}%
% \def\Titlefont{\reset@font\fontsize{17bp}{22.5bp}\selectfont\titraggedcenter}%
% \def\SubTitlefont{\reset@font\fontsize{14bp}{16.5bp}\selectfont\titraggedcenter}%
% \def\Authorfont{\reset@font\fontsize{12bp}{14.5bp}\selectfont\boldmath\titraggedcenter}%
% \def\addressfont{\reset@font\fontsize{11bp}{13.5bp}\selectfont\titraggedcenter}%
% \def\abstractheadfont{\reset@font\fontsize{9bp}{11bp}\bfseries\selectfont\titraggedcenter}%
% \def\abstractsubheadfont{\reset@font\fontsize{9bp}{11bp}\bfseries\selectfont}%
% \def\abstractfont{\reset@font\fontsize{9bp}{11bp}\selectfont\leftskip=24pt\rightskip=24pt\parfillskip=0pt plus 1fil}%
% \def\keywordfont{\reset@font\fontsize{8bp}{9.5bp}\selectfont\leftskip=24pt\rightskip=24pt plus0.5fill}%
% \def\historyfont{\reset@font\fontsize{8bp}{9.5bp}\selectfont\leftskip=24pt\rightskip=24pt plus0.5fill}%

% %% Article Type

% \newbox\artcatbox%



% \def\articletype#1{\if!#1!\else\setbox\artcatbox\hbox{\Artcatfont\hskip1mm#1\hskip1mm}\fi%
% \gdef\ArtType{\fboxsep=0pt{\vbox to 4mm{\vfil%
%               {\raggedright\box\artcatbox}\vfil}}}%
% \gdef\@ArtType{#1}}%
% %%\articletype{RESEARCH ARTICLE}%
% \articletype{}%


% %% Article Title

% \renewcommand{\title}[2][]{%
% \gdef\@checktitle{#1}\ifx\@checktitle\empty\gdef\@title{#2}%
% \gdef\s@title{#2}\else\gdef\@title{#2}\gdef\s@title{#1}\fi%
% \markboth{\textit{\s@title}}{\textit{\s@title}}}%

% \def\subtitle#1{\gdef\@subtitle{#1}}\subtitle{}%

% %% Cross Link for Author & Address
% \def\jmkLabel#1{\@bsphack\protected@write\@auxout{}{\string\Newlabel{#1}{\@currentlabel}}\@esphack}%
% \def\Newlabel#1#2{\expandafter\xdef\csname X@#1\endcsname{#2}}%
% \def\jmkRef#1{\@ifundefined{X@#1}{0}{\csname X@#1\endcsname}}%

% %% Article Author(s)
% \let\sep\@empty%
% \let\authorsep\@empty%
% \newcount\aucount%
% \newcount\corraucount%
% \newcount\punctcount%
% %
% \def\artauthors{}%
% \newif\if@auemail%
% \newif\if@corauemail%
% %
% \def\au@and{\ifnum\punctcount=2\ and\else\unskip, \advance\punctcount by -1 \fi}%
% %
% \def\author{\advance\aucount by 1\@ifstar\@@corrauthor\@@author}%
% %
% \newcommand{\@@author}[2][]{\def\@authfrstarg{#1}\@corauemailfalse%
% \g@addto@macro\artauthors{%
%     \ifnum\aucount=1%
%     \global\@auemailtrue%
%     \else%
%     \global\@auemailfalse%
%     \fi%
%     \Authorfont%
%     \def\baselinestretch{1}%
%     \authorsep{#2}\unskip\ifx\@authfrstarg\empty\else\textsuperscript{\smash{{%
%       \@for\@@affmark:=#1\do{\edef\affnum{\@ifundefined{X@\@@affmark}{\@@affmark}{\jmkRef{\@@affmark}}}%
%      \unskip\sep\affnum\let\sep=,}}}}\fi%
%     \def\authorsep{{\au@and} }%%% 
%     \global\let\sep\@empty\global\let\@corref\@empty%
% }}%
% %
% \newcommand{\@@corrauthor}[2][]{\def\@authfrstarg{#1}\@corauemailtrue\advance\corraucount by 1%
% \g@addto@macro\artauthors{%
%     \global\@auemailtrue%
%     \Authorfont%
%     \def\baselinestretch{1}%
%     \authorsep{#2}\unskip\ifx\@authfrstarg\empty\else\textsuperscript{\smash{{%
%       \@for\@@affmark:=#1\do{\edef\affnum{\@ifundefined{X@\@@affmark}{\@@affmark}{\jmkRef{\@@affmark}}}%
%      \unskip\sep\affnum\let\sep=,}}}{*}\hskip-1pt}\fi\unskip%
%     \def\authorsep{\au@and~}%%% 
%     \global\let\sep\@empty\global\let\@corref\@empty%
% }}%
% %%
% %% Miscellaneous macros %%
% %%
% \def\fnm#1{\leavevmode\hbox{#1}}%
% \def\sur#1{\unskip~\nobreak\leavevmode\hbox{#1}}%
% \def\spfx#1{#1}%
% \def\pfx#1{#1}%
% \def\sfx#1{#1}%
% \def\tanm#1{#1}%
% \def\dgr#1{#1}%
% %
% %% Author Email
% %
% \let\nomail\relax%
% \def\corrauthemail{}%
% \def\authemail{}%

% \newcount\emailcnt%

% \def\email#1{\global\advance\emailcnt by 1\relax%
% \if@corauemail%
%    \g@addto@macro\corrauthemail{%
%    \setcounter{footnote}{0}%
%    \textcolor{blue}{#1};\ %
%    }%
% \else%
%    \g@addto@macro\authemail{%
%    \setcounter{footnote}{0}%
%    \textcolor{blue}{#1};\ %
%    }%
% \fi}

% %% Corrseponding Address 
% \def\@copycorthanks{}%
% \def\auaddress{}%
% \def\@auaddress{}%

% \newcounter{affn}%
% \newcount\addcount% To check the count of address

% \renewcommand\theaffn{\arabic{affn}}%

% \def\affil{\advance\addcount by 1\@ifstar\@@coraddress\@@address}%

% \newcommand{\@@coraddress}[2][]{%\advance\addcount by 1
% \g@addto@macro\auaddress{%
%      \stepcounter{affn}%
%      \xdef\@currentlabel{\theaffn}%
%      \jmkLabel{\theaffn}%
%      {\textsuperscript{#1*}#2.\par} }
% }

% %% Macros for present address

% \newif\ifpresentaddress%

% \def\@presentaddresstxt{}% 
% \def\presentaddresstxt#1{\gdef\@presentaddresstxt{#1:}}\presentaddresstxt{Present Address}%
% \newcommand{\presentaddress}[1]{\gdef\@presentaddresstext{\@presentaddresstxt\par#1}\global\presentaddresstrue}%

% %% Macros for equally contributed

% \newif\ifequalcont%

% %\def\@equalconttxt{}% 
% %\def\equalcontxt#1{\gdef\@equalconttxt{#1}}\equalcontxt{These authors contributed equally to this work.}%
% %\newcommand{\equalcont}[1][\@equalconttxt]{\gdef\@equalconttext{#1}\g@addto@macro\artauthors{$^{\dagger}$}\global\equalconttrue}%

% \def\@equalconttxt{}% 
% \def\equalcontxt#1{\gdef\@equalconttxt{#1}}\equalcontxt{}%
% \newcommand{\equalcont}[1]{\gdef\@equalconttext{#1}\g@addto@macro\artauthors{$^{\dagger}$}\global\equalconttrue}%

% %% Author Address 

% \newcommand{\@@address}[2][]{%%\advance\addcount by 1
% \g@addto@macro\auaddress{%
%      \stepcounter{affn}%
%      \xdef\@currentlabel{\theaffn}%
%      \jmkLabel{\theaffn}%
%      {\textsuperscript{#1}#2.\par} }%\theaffn
% }

% %% Address tagging 
% \newcommand{\orgdiv}[1]{#1}%
% \newcommand{\orgname}[1]{#1}%
% \newcommand{\orgaddress}[1]{#1}%
% \newcommand{\street}[1]{#1}%
% \newcommand{\postcode}[1]{#1}%
% \newcommand{\city}[1]{#1}%
% \newcommand{\state}[1]{#1}%
% \newcommand{\country}[1]{#1}%

% %% Article notes

% \def\@artnote{}%
% \def\artnote#1{\gdef\@artnote{#1}}%

% %% Miscellaneous notes 

% \def\@miscnote{}%
% \def\miscnote#1{\gdef\@miscnote{\par\addvspace{3pt}#1}}%

% %% Motto

% \def\mottofont{\reset@font\fontfamily{\rmdefault}\fontsize{8.5bp}{10bp}\fontshape{it}\selectfont\raggedright}
% %
% \let\@motto\@empty
% \def\mottoraggedright{\rightskip0mm\leftskip=42mm plus 1fil\parfillskip=0pt\relax}%
% \newcommand{\motto}[2][]{\gdef\@headcheck{#1}\gdef\@motto{\@headcheck\ifx\@headcheck\@empty\vskip12pt\else\fi{\mottofont\mottoraggedright#2\par}}}

% %% Article Abstract
% \newcommand\abstracthead{\@startsection {section}{1}{\z@}{-22pt \@plus0ex \@minus0ex}{3pt}{\abstractheadfont}}
% \newcommand\subabstracthead{\@startsection{subsection}{2}{\z@}{3pt \@plus0ex \@minus0ex}{-.5em}{\abstractsubheadfont}}

% \def\@abstract{}%
% \long\def\abstract#1{\def\@abstract{%
% \let\paragraph\subabstracthead%
% \abstractfont%
% \abstracthead*{\abstractname}%
% #1\par}}%

% \def\printabstract{\ifx\@abstract\empty\else\@abstract\fi\par}%

% \def\printkeywords{\ifx\@keywords\empty\else\@keywords\fi\par}%

% %
% %% Keywords
% \def\keywordname{Keywords}%
% \def\keywords#1{\ifx#1\empty\else\def\@keywords{\par\addvspace{10pt}{\keywordfont{\bfseries\keywordname:} #1\par}}\fi}%
% \def\@keywords{}%

% %% PACs

% \def\pacsbullet{\hbox{\hskip2.5pt,\hskip2.5pt}}%

% \def\change@commas#1,#2{%
%   \ifx#2\@empty%
%     #1%
%   \else%
%     #1\nobreak\hbox{\pacsbullet}\allowbreak\expandafter\change@commas%
%   \fi%
%   #2}%

% \newcommand\keywordhead[1]{\par\addvspace{10pt}%
% {{\keywordfont\bfseries#1:\ }}}%

% \newcommand{\pacs}[1]{\keywordhead{\pacsname}#1}%
% %
% \newcount\PacsCount%
% \PacsCount=0%
% %
% \newcount\PacsTmpCnt%
% \PacsTmpCnt=1%
% %
% \gdef\StorePacsText#1#2{%
% \edef\GetRoman{\romannumeral#1}%
% \expandafter\gdef\csname\GetRoman StorePacsTxt\endcsname{#2}%
% }%
% %
% \let\oldpacs\pacs%
% \renewcommand\pacs[2][PAC Codes]{\gdef\pacsname{{\bfseries#1}}\gdef\@pacs{\keywordfont\raggedright\oldpacs\change@commas#2,\@empty\par}
% \StepUpCounter{\PacsCount}%
% \StorePacsText{\the\PacsCount}{\gdef\pacsname{{\bfseries#1}}\keywordfont\raggedright\oldpacs\change@commas#2,\@empty}%
% }%

% \def\@pacs{}%

% %% Glossary

% \def\gloshead{Glossary}%

% \newenvironment{glos}[1][\gloshead]{\begingroup\parindent=0pt%
% \section*{#1}
% \def\item[##1]{##1,\ }}{%
% \endgroup}%
% %

% %% Article History

% \def\received#1{\g@addto@macro\@history{{Received #1}}}%
% \def\revised#1{\g@addto@macro\@history{{; revised #1}}}%
% \def\accepted#1{\g@addto@macro\@history{{; accepted #1}}}%

% %% Remark on Front page %%

% \newdimen\FMremarkdim%

% \newcommand{\FMremark}{\begingroup\parindent=0pt\parskip=0pt%
% \if@referee\singlespacing\fi%
% \fboxsep=6pt\fboxrule=0.5pt%
% \FMremarkdim=\textwidth%%\paperwidth%
% \advance\FMremarkdim-\fboxsep%
% \advance\FMremarkdim-2\fboxrule%
% \if@referee\vskip-21pt\fi%
% %%\fbox{\vbox{\hsize=\FMremarkdim\small%
% \unvbox\fmremarkbox
% %%}}%
% \endgroup}

% \newbox\fmremarkbox%

% \newenvironment{fmremark}{\begingroup\parindent=0pt%
% \fboxsep=6pt\fboxrule=0.5pt%
% \FMremarkdim=\textwidth%%\paperwidth%
% \advance\FMremarkdim-\fboxsep%
% \advance\FMremarkdim-2\fboxrule%
% \global\setbox\fmremarkbox\vbox\bgroup\small%
% }{\egroup\endgroup}

% %% Article Header Definition
% \renewcommand{\@maketitle}{\newpage\null%
%     \if@remarkboxon\vbox to 0pt{\vspace*{-78pt}\hspace*{-18pt}\FMremark}\else\vskip21pt\fi%%\par%
%     \hsize\textwidth\parindent0pt%%%\vskip7pt%
%     %% Aritle Type
%     {\hbox to \textwidth{{\Artcatfont\ArtType\hfill}\par}}
%     %% Aritle Title
%     \ifx\@title\empty\else%
%         \removelastskip\vskip20pt\nointerlineskip%
%         {\Titlefont\@title\par}
%         %\addcontentsline{toc}{chapter}{\@title}% for bookmarks
%     \fi%
%     %% Aritle SubTitle
%     \ifx\@subtitle\empty\else%
%         \vskip9pt%
%         {{\SubTitlefont\@subtitle\par}}
%     \fi%
%     %% Aritle Authors, Address and Correspondings
%     \ifnum\aucount>0
%         \global\punctcount\aucount%
%         \vskip20pt%
%         \artauthors\par%%     authors and emails
%         {\vskip7pt\addressfont\auaddress\par%%      corresponding adress
% 	 \removelastskip\vskip24pt%
% 	\ifnum\emailcnt>0\relax%
%            \ifx\corrauthemail\@empty\else{\ifnum\aucount>1*\fi}%
% 	   Corresponding author(s). E-mail(s): \corrauthemail\par\fi%
% 	   \ifx\authemail\@empty\else Contributing authors:\ \authemail\fi%
%         \fi%
%         \ifequalcont{\par$^{\dagger}$\@equalconttext\par}\fi%
% 	 \removelastskip\vskip24pt%
%         \ifpresentaddress{\par\@presentaddresstext\par}\fi%
% 	}
%      \fi%
%      {\printabstract\par}%
%      {\printkeywords\par}%
%      \ifx\@pacs\empty\else%
%        \loop\ifnum\PacsCount>0%
%           \csname\romannumeral\PacsTmpCnt StorePacsTxt\endcsname\par%
%           \StepDownCounter{\PacsCount}%
%           \StepUpCounter{\PacsTmpCnt}%
%        \repeat%
%     \fi%
%     %%{\printhistory\par}%
%     %%{\ifx\@motto\empty\else\@motto\fi}%
%     \removelastskip\vskip36pt\vskip0pt}%

% \usepackage{cuted}%
% \@ifpackageloaded{cuted}{\gdef\@setmarks{}}{}%

% %% Printing Article Header
% \newdimen\firstpagehtcheck

% \renewcommand\maketitle{\par
%   \@afterindentfalse%
%   \begingroup
%     \gdef\UrlFont{\rmfamily}%
%     \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
%     \def\@makefnmark{\rlap{\@textsuperscript{\normalfont\smash{\@thefnmark}}}}%
%     \long\def\@makefntext##1{\parindent 1em\noindent\small\selectfont
%             \hbox{\@textsuperscript{\normalfont\@thefnmark}}##1}%
%     \if@twocolumn
%       \ifnum \col@number=\@ne%
% \setbox0=\vbox{\@maketitle}
% \firstpagehtcheck=\ht0%
% \advance\firstpagehtcheck by \dp0%
% \ifdim\firstpagehtcheck>\textheight%
% \setbox1=\vsplit0to2\textheight%
% \setbox1=\vbox{\unvbox1}%
% \setbox2=\vbox{\unvbox0}%
% \unvbox1%
% \stripsep=0pt%
% \begin{strip}
% \unvbox2%
% \end{strip}
% \else
% \twocolumn[\@maketitle]%
% \fi      
% \else
% \@maketitle
% \fi%
%     \else%
%       \newpage%
%       \global\@topnum\z@% Prevents figures from going at top of page.
%       \@maketitle%
%     \fi%
%   \endgroup%
%   \ifx\@artnote\@empty\else\footnoteA{\@artnote}\fi%
%   \ifx\@miscnote\@empty\else\footnoteA{\@miscnote\par}\fi%
%   \setcounter{footnote}{0}%
%   \global\let\thanks\relax%
%   \global\let\artnote\relax%
%   \global\let\maketitle\relax%
%   \global\let\@maketitle\relax%
%   \global\let\@thanks\@empty%
%   \global\let\@author\@empty%
%   \global\let\@date\@empty%
%   \global\let\title\relax%
%   \global\let\author\relax%
%   \global\let\date\relax%
%   \global\let\and\relax%
%   \pagestyle{headings}%
%   %%%print continuous abstract on next page
%   \@afterheading%
%   %%\vskip-18pt% this is included to avoid vertical space at the beginning of left column on article opening pages
% }%

% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Page Styles %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% %
% \def\opheaderfont{\reset@font\fontsize{10bp}{0bp}\selectfont}%
% \def\headerfont{\reset@font\fontsize{10bp}{0bp}\selectfont}%
% \def\footerfont{\reset@font\fontsize{10bp}{0bp}\selectfont}%

% %% Regular Page Style      
% \def\ps@headings{%
%     \def\@oddfoot{\hfill\thepage\hfill}%
%     \let\@evenfoot\@oddfoot%
%       \def\@evenhead{%
%       \vbox to 0pt{\vspace*{-48pt}%
%          \hbox to \hsize{\hfill \relax\hfill}}\par%%
%       \hspace*{-\textwidth}\hbox to \hsize{\hfill}}%
%       \def\@oddhead{%
%       \vbox to 0pt{\vspace*{-48pt}%
%          \hbox to \hsize{\hfill \relax\hfill}}\par%%
%       \hspace*{-\textwidth}\hbox to \hsize{\hfill}}%
%       \let\@mkboth\markboth%
%       }%


% %% Opening Page Style      
% \def\ps@titlepage{%
%      %%\def\@oddhead{\vbox{\vskip-36pt\hbox to \textwidth{\hfill\includegraphics{springer-nature-logo}\hspace*{-1pt}}}}%
%      %%\let\@oddhead\@empty\let\@evenhead\@empty%
%       \def\@oddhead{%
%       \vbox to 0pt{\vspace*{-38pt}%
%          \hbox to \hsize{\hfill \hfill}}}%%
%      \let\@evenhead\@oddhead%
%      \def\@oddfoot{\vbox to 18pt{\vfill\reset@font\rmfamily\hfil\thepage\hfil}}%%
%      \def\@evenfoot{}}%

% \def\ps@plain{\let\@mkboth\@gobbletwo%
% \let\@oddhead\@empty\let\@evenhead\@empty%
% \def\@oddfoot{\vbox to 18pt{\vfill\reset@font\rmfamily\hfil ddd\thepage\hfil}}%
% \let\@evenfoot\@oddfoot}%

% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Sections %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %

% \def\numbered{\setcounter{secnumdepth}{3}}%
% \def\unnumbered{\setcounter{secnumdepth}{0}}%
% \numbered%% default is numbered Sections

% \renewcommand\thesection      {\@arabic\c@section}%
% \renewcommand\thesubsection   {\thesection.\@arabic\c@subsection}%
% \renewcommand\thesubsubsection{\thesubsection.\@arabic\c@subsubsection}%
% \renewcommand\theparagraph    {\thesubsubsection.\@arabic\c@paragraph}%
% \renewcommand\thesubparagraph {\theparagraph.\@arabic\c@subparagraph}%
% %%
% \def\@seccntformat#1{\csname the#1\endcsname\hskip.5em}%

% \def\@sect#1#2#3#4#5#6[#7]#8{%
%   \ifnum #2>\c@secnumdepth
%     \let\@svsec\@empty
%   \else
%     \refstepcounter{#1}%
%       \protected@edef\@svsec{\@seccntformat{#1}\relax}%
%   \fi
%   \@tempskipa #5\relax
%   \ifdim \@tempskipa>\z@
%     \begingroup
%       #6{%
%         \@hangfrom{\hskip #3\relax\@svsec}%
%           \interlinepenalty \@M #8\@@par}%
%     \endgroup
%     \csname #1mark\endcsname{#7}%
%     \addcontentsline{toc}{#1}{%
%       \ifnum #2>\c@secnumdepth \else
%         \protect\numberline{\csname the#1\endcsname}%
%       \fi
%       #7}%
%   \else
%     \def\@svsechd{%
%       #6{\hskip #3\relax
%       \@svsec #8.}%
%       \csname #1mark\endcsname{#7}%
%       \addcontentsline{toc}{#1}{%
%         \ifnum #2>\c@secnumdepth \else
%           \protect\numberline{\csname the#1\endcsname}%
%         \fi
%         #7}}%
%   \fi
%   \@xsect{#5}}
% %
% \def\sectionfont{\reset@font\fontfamily{\rmdefault}\fontsize{14bp}{16bp}\bfseries\selectfont\raggedright\boldmath}%
% \def\subsectionfont{\reset@font\fontfamily{\rmdefault}\fontsize{12bp}{14bp}\bfseries\selectfont\raggedright\boldmath}%
% \def\subsubsectionfont{\reset@font\fontsize{11bp}{13bp}\bfseries\selectfont\raggedright\boldmath}%
% \def\paragraphfont{\reset@font\fontsize{10bp}{12bp}\bfseries\itshape\selectfont\raggedright}%
% %
% \def\subparagraphfont{\itshape}%
% \def\bmheadfont{\reset@font\fontfamily{\rmdefault}\fontsize{10bp}{12bp}\bfseries\selectfont\raggedright\boldmath}%
% %
% \renewcommand\section{\@startsection{section}{1}{\z@}%
%                                     {-12pt \@plus -4pt \@minus -2pt}%
%                                     {9pt}%
%                                     {\sectionfont}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                        {-12pt \@plus -4pt \@minus -2pt}%
%                                        {6pt}%
%                                        {\subsectionfont}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                           {-12pt \@plus -4pt \@minus -2pt}%
%                                           {6pt}%
%                                           {\subsubsectionfont}}
% \renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
%                                       {-12pt \@plus -4pt \@minus-2pt}%
%                                       {3pt}%
%                                       {\paragraphfont}}
% \renewcommand\subparagraph{\@startsection{subparagraph}{5}{\z@}%
%                                          {6pt \@plus1ex \@minus.2ex}%
%                                          {-1em}%
%                                          {\subparagraphfont}}
% \newcommand\bmhead{\@startsection{subparagraph}{5}{\z@}%
%                                  {6pt \@plus1ex \@minus .2ex}%
%                                  {-1em}%
%                                  {\bmheadfont}}
% %
% \def\@startsection#1#2#3#4#5#6{%
%   \if@noskipsec \leavevmode \fi
%   \par
%   \@tempskipa #4\relax
%   \@afterindenttrue
%   \ifdim \@tempskipa <\z@
%     \@tempskipa -\@tempskipa \@afterindentfalse
%   \fi
%   \if@nobreak
%     \everypar{}%
%   \else
%     \addpenalty\@secpenalty\addvspace\@tempskipa
%   \fi
%   \@ifstar
%     {\@ssect{#3}{#4}{#5}{#6}}%
%     {\@dblarg{\@sect{#1}{#2}{#3}{#4}{#5}{#6}}}}
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Lists %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% \newdimen\labelwidthi%
% \newdimen\labelwidthii%
% \newdimen\labelwidthiii%
% \newdimen\labelwidthiv%

% \def\normal@labelsep{0.5em}%
% \labelsep\normal@labelsep%
% \settowidth{\labelwidthi}{(iii)}%
% \settowidth{\labelwidthii}{(d)}%
% \settowidth{\labelwidthiii}{(iii)}%
% \settowidth{\labelwidthiv}{(M)}%

% \leftmargini\labelwidthi     \advance\leftmargini\labelsep
% \leftmarginii\labelwidthii   \advance\leftmarginii\labelsep
% \leftmarginiii\labelwidthiii \advance\leftmarginiii\labelsep
% \leftmarginiv\labelwidthiv   \advance\leftmarginiv\labelsep

% \def\setleftmargin#1#2{\settowidth{\@tempdima}{#2}\labelsep\normal@labelsep
%   \csname labelwidth#1\endcsname\@tempdima
%   \@tempdimb\@tempdima \advance\@tempdimb\labelsep
%   \csname leftmargin#1\endcsname\@tempdimb}
% \def\@listI{\leftmargin\leftmargini
%   \labelwidth\labelwidthi \labelsep\normal@labelsep
% %  \topsep \z@ 
%   \topsep\baselineskip %%updated
%   \partopsep\z@ \parsep\z@ \itemsep\z@
%   \listparindent 1em}
% \def\@listii{\leftmargin\leftmarginii
%   \labelwidth\labelwidthii \labelsep\normal@labelsep
%   \topsep\z@ \partopsep\z@ \parsep\z@ \itemsep\z@
%   \listparindent 1em}
% \def\@listiii{\leftmargin\leftmarginiii
%   \labelwidth\labelwidthiii \labelsep\normal@labelsep
%   \topsep\z@ \partopsep\z@ \parsep\z@ \itemsep\z@
%   \listparindent 1em}
% \def\@listiv{\leftmargin\leftmarginiv
%   \labelwidth\labelwidthiv \labelsep\normal@labelsep
%   \topsep\z@ \partopsep\z@ \parsep\z@ \itemsep\z@
%   \listparindent 1em}
% \let\@listi\@listI
% \@listi
% %
% \setlength  \labelsep  {.5em}
% \setlength  \labelwidth{\leftmargini}
% \addtolength\labelwidth{-\labelsep}
% \@beginparpenalty -\@lowpenalty
% \@endparpenalty   -\@lowpenalty
% \@itempenalty     -\@lowpenalty
% \def\labelitemi{$\bullet$}          \def\labelitemii{$\cdot$}
% \def\labelenumi{\theenumi.}         \def\theenumi{\arabic{enumi}}
% \def\labelenumii{(\alph{enumii})}   \def\theenumii{\alph{enumii}}
% \def\labelenumiii{(\roman{enumiii})}\def\theenumiii{\roman{enumiii}}
% \def\labelenumiv{(\Alph{enumiv})}   \def\theenumiv{\Alph{enumiv}}

% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%% Ordered & Unordered List  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% \def\listfont{\normalsize}%
% %
% \def\enumargs{%
%    \listfont%
%    \leftmargini0pt%
%    \leftmarginii0pt%
%    \leftmarginiii0pt%
%    \ifnum\@enumdepth=3\topsep0pt\else\ifnum\@enumdepth=2\topsep0pt\else\topsep 6pt\fi\fi%
%    \partopsep     \z@%
%    \itemsep       \z@%
%    \parsep        \z@%
%    \labelsep      0.5em%
%    \rightmargin   \z@%
%    \raggedright%   
%    \listparindent \parindent%
%    \itemindent    \z@}%

% \def\enumerate{%
%     \@ifnextchar[{\@numerate}{\@numerate[0.]}}

% \def\@numerate[#1]{\par%
%      \ifnum \@enumdepth >3 \@toodeep\else
%      \advance\@enumdepth \@ne
%      \edef\@enumctr{enum\romannumeral\the\@enumdepth}
%      \list{\csname label\@enumctr\endcsname}{%
%        \enumargs%
%        \setlength{\leftmargin}{\csname leftmargin\romannumeral\the\@enumdepth\endcsname}
%        \usecounter{\@enumctr}
%        \settowidth\labelwidth{#1}
%        \addtolength{\leftmargin}{\labelwidth}
%        \addtolength{\leftmargin}{\labelsep}
%        \def\makelabel##1{\hss\llap{##1}}}%
%      \fi
%    }
% \let\endenumerate\endlist

% %%Unnumbered list%%

% \def\unenumargs{%
%    \listfont%
%    \leftmargini\parindent%
%    \topsep6pt%
%    \partopsep     \z@%
%    \itemsep       \z@%
%    \parsep        \z@%
%    \labelsep      0\p@%
%    \rightmargin   \z@%
%    \raggedright%
%    \listparindent \parindent%
%    \itemindent    -12pt}%

% \def\unenumerate{%
%     \@ifnextchar[{\@unenumerate}{\@unenumerate[0.]}}

% \def\@unenumerate[#1]{\par%
%      \ifnum \@enumdepth >3 \@toodeep\else
%      \advance\@enumdepth \@ne
%      \edef\@enumctr{enum\romannumeral\the\@enumdepth}
%      \list{}{%
%        \unenumargs
%        \setlength{\leftmargin}{\csname leftmargin\romannumeral\the\@enumdepth\endcsname}
%        \usecounter{\@enumctr}
%        \settowidth\labelwidth{#1}
%        \addtolength{\leftmargin}{0pt}
%        \addtolength{\leftmargin}{0pt}
%        \def\makelabel##1{\hss\llap{##1}}}%
%      \fi
%    }

% \let\endunenumerate\endlist%

% %% bulleted list 

% \def\itemargs{%
%    \listfont%
%    \leftmargini0pt%
%    \leftmarginii0pt%
%    \ifnum\@enumdepth=3\topsep0pt\else\ifnum\@enumdepth=2\topsep0pt\else\topsep 6pt\fi\fi%
%    \partopsep     \z@%
%    \itemsep       \z@%
%    \parsep        \z@%
%    \labelsep      0.5em%
%    \rightmargin   \z@%
%    \raggedright%
%    \listparindent \z@%
%    \itemindent    \z@}%

% \renewcommand\labelitemi{\raise1pt\hbox{\textbullet}}%
% \renewcommand\labelitemii{\textendash}%

% \def\itemize{%
%    \@ifnextchar[{\@itemize}{\@itemize[$\bullet$]}}

% \def\@itemize[#1]{\par%
%      \ifnum \@itemdepth >3 \@toodeep\else
%      \advance\@itemdepth \@ne
%      \edef\@itemctr{item\romannumeral\the\@itemdepth}
%      \list{\csname label\@itemctr\endcsname}{%
%        \itemargs
%        \setlength{\leftmargin}{\csname leftmargin\romannumeral\the\@itemdepth\endcsname}
%        \settowidth\labelwidth{#1}
%        \addtolength{\leftmargin}{\labelwidth}
%        \addtolength{\leftmargin}{\labelsep}
%        \def\makelabel##1{\hss \llap{##1}}}%
%      \fi
%    }
% \let\enditemize\endlist
% %
% \def\quote{\list{}{\itemindent\z@
%    \leftmargin 1em \rightmargin \z@}%
% \item[]}
% \let\endquote\endlist
% %
% \def\descriptionlabel#1{\hspace\labelsep \itshape #1}
% \def\description{\list{}{\labelwidth\z@
%   \leftmargin \z@ \topsep6pt\itemindent \z@ %-\leftmargin
%   \let\makelabel\descriptionlabel}}
% \let\enddescription\endlist

% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Float %%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \setlength\abovecaptionskip{2.25\p@}%
% \setlength\belowcaptionskip{6\p@}%

% \setlength\arraycolsep{2\p@}%
% \setlength\tabcolsep{6\p@}%
% \setlength\arrayrulewidth{.4\p@}%
% \setlength\doublerulesep{2\p@}%
% \setlength\tabbingsep{\labelsep}%

% \def\fnum@figure{{\bfseries\figurename\space\thefigure}}%
% \def\fnum@table{{\bfseries\tablename\space\thetable}}%

% \def\FigName{figure}%

% \long\def\@makecaption#1#2{%
%     \ifx\FigName\@captype
%       \vskip\abovecaptionskip
%         \@figurecaption{#1}{#2}
%     \else
%         \@tablecaption{#1}{#2}
%       \vskip\belowcaptionskip
%     \fi%
% }

% %% Figure

% \def\figurecaptionfont{\reset@font\fontfamily{\rmdefault}\fontsize{8}{9.5}\selectfont}%

% \newdimen\figwidth%
% \newdimen\figheight%
% \newdimen\sidecapwidth
% \newdimen\wrapcapline%
% \newdimen\totalwrapline%
% \newdimen\wraptotline%

% %% Figures macro
% \newbox\figurebox%
% \newbox\wrapfigcapbox

% \def\FIG#1#2{%
% \setbox\figurebox\hbox{#1}%
% %% Figure dimensions
% \figwidth\wd\figurebox%
% \figheight\ht\figurebox%
% {\parbox{\hsize}{%
% \centerline{\box\figurebox}%
% %% Caption
% #2}}}

% %% Figures caption
% \newbox\figcapbox
% \newbox\capbox
% \long\def\@figurecaption#1#2{{\figurecaptionfont{\bfseries#1}\hskip.7em#2\par}}%

% \newenvironment{unnumfigure}{\begingroup\setlength{\topsep}{12pt}%
% \begin{center}}{\end{center}\endgroup}

% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% \@ifpackageloaded{booktabs}{\cmidrulewidth=.15pt}{}%
% %
% \def\tablecaptionfont{\reset@font\fontsize{8bp}{9.5bp}\selectfont}%
% \def\tablebodyfont{\reset@font\fontsize{8bp}{9.5bp}\selectfont}%
% \def\tablecolheadfont{\reset@font\fontsize{8bp}{9.5bp}\selectfont\bfseries\boldmath}%
% \def\tablefootnotefont{\reset@font\fontsize{8bp}{9.5bp}\selectfont}%

% %% Table Macro

% \newskip\headwidthskip%

% \def\tabraggedcenter{\leftskip=0pt plus 0.5fil\rightskip=0pt plus 0.5fil\parfillskip=0pt}%

% \newenvironment{@processtable}[4]{%
% \setbox4=\hbox to \hsize{\hss%
% \begin{minipage}[t]{#4}%
% \tabraggedcenter%
% \caption{#1}\par%
% {\tablebodyfont\noindent\ignorespaces#2\par}\par\vglue6pt%
% {\if!#3!\else{\tablefootnotefont#3}\fi}%
% \end{minipage}%
% \hss}%
% \box4\par}%

% \newcommand\TBL[3]{\begingroup%
% %
% \if!#1!\let\caption\relax\fi%
% %
%    \global\setbox\temptbox=\hbox{\bgroup{\tablebodyfont#2}\egroup}%
%    \global\tempdime\wd\temptbox%
%     \@processtable{#1}{\global\headwidthskip=\tempdime%
% 	 \vbox{#2}}{#3}{\tempdime}%
% \endgroup}%

% %% Table Caption
% \newbox\tabcapbox%
% \newbox\temptbox%
% \newdimen\tempdime%
% \newdimen\tabhtdime%

% \long\def\@tablecaption#1#2{%
%   \setbox\tabcapbox\vbox{\tablecaptionfont\raggedright%
%   {\bfseries #1}{\hskip2mm}#2\vphantom{y}\par}%
%   \box\tabcapbox%
% }

% %% Table Column Heads
% \def\TCH#1{{\tablecolheadfont #1}}

% %% Table Footnotes

% \newenvironment{tablenotes}{\list{}{\setlength{\labelsep}{0pt}% 
% \setlength{\labelwidth}{0pt}%
% \setlength{\leftmargin}{0pt}%
% \setlength{\rightmargin}{0pt}%
% \setlength{\topsep}{-6pt}%
% \setlength{\itemsep}{2pt}%
% \setlength{\partopsep}{0pt}%
% \setlength{\listparindent}{0em}%
% \setlength{\parsep}{0pt}}%
% \item\relax%
% }{\endlist}%

% \def\tnote#1{$^{#1}$}%%

% %% Table Rules

% \def\toprule{%\noalign{\vskip3pt}
% \noalign{\ifnum0=`}\fi
%   \hrule \@height 0\p@ \@width 0pt
%   \hrule \@height 0.75\p@ % <- rule height
%   \hrule \@height 5pt \@width 0pt
%   \futurelet\@tempa\@xhline}
% % Middle rule
% \def\midrule{\noalign{\ifnum0=`}\fi%
%   \hrule \@height 3pt \@width 0pt
%   \hrule \@height .5pt % <- rule height
%   \hrule \@height 5pt \@width 0pt
%   \futurelet \@tempa\@xhline}
% % Bottom rule
% \def\botrule{\noalign{\ifnum0=`}\fi
%   \hrule \@height 3pt \@width 0pt
%   \hrule \@height 0.75\p@ % <- rule height
%   \hrule \@height 3pt \@width 0pt
%   \futurelet\@tempa\@xhline}
% %
% \def\@@@cmidrule[#1-#2]#3#4{\global\@cmidla#1\relax
%     \global\advance\@cmidla\m@ne
%     \ifnum\@cmidla>0\global\let\@gtempa\@cmidrulea\else
%     \global\let\@gtempa\@cmidruleb\fi
%     \global\@cmidlb#2\relax
%     \global\advance\@cmidlb-\@cmidla
%     \global\@thisrulewidth=#3
%     \@setrulekerning{#4}
%     \ifnum\@lastruleclass=\z@\vskip 3\p@\fi
%     \ifnum0=`{\fi}\@gtempa
%     \noalign{\ifnum0=`}\fi\futurenonspacelet\@tempa\@xcmidrule}
% \def\@xcmidrule{%
%    \ifx\@tempa\cmidrule
%        \vskip-\@thisrulewidth
%        \global\@lastruleclass=\@ne
%    \else \ifx\@tempa\morecmidrules
%        \vskip \cmidrulesep
%        \global\@lastruleclass=\@ne\else
%        \vskip 5\p@
%        \global\@lastruleclass=\z@
%    \fi\fi
%    \ifnum0=`{\fi}}
% \let\cline\cmidrule

% \usepackage[figuresright]{rotating}%
% \usepackage{threeparttable}

% \let\tableorg\table%
% \let\endtableorg\endtable%

% \let\sidewaystableorg\sidewaystable%
% \let\endsidewaystableorg\endsidewaystable%

% \renewenvironment{table}[1][]%
% {\begin{tableorg}[#1]%
% \begin{center}
% \begin{threeparttable}
% \tablebodyfont%
% \renewcommand\footnotetext[2][]{{\removelastskip\vskip3pt%
% \let\tablebodyfont\tablefootnotefont%
% \hskip0pt\if!##1!\else{\smash{$^{##1}$}}\fi##2\par}}%
% }{\end{threeparttable}\end{center}\end{tableorg}}

% \renewenvironment{sidewaystable}[1][]%
% {\begin{sidewaystableorg}[#1]%
% \begin{center}
% \begin{threeparttable}
% \tablebodyfont%
% \renewcommand\footnotetext[2][]{{\removelastskip\vskip3pt%
% \let\tablebodyfont\tablefootnotefont%
% \hskip0pt\if!##1!\else{\smash{$^{##1}$}}\fi##2\par}}%
% }{\end{threeparttable}\end{center}\end{sidewaystableorg}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%% Other Env. %%%%%%%%%%%%%%%%%%%%%%%%%

% \def\quotefont{\reset@font\fontfamily{\rmdefault}\fontsize{9}{11}\selectfont}%

% \renewenvironment{quote}
%                {\list{}{\topsep=0pt\topsep6pt\leftmargin=1em\raggedright\quotefont}%
%                 \item\relax}
%                {\endlist}
               
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%% Appendix %%%%%%%%%%%%%%%%%%%%%%%%%
% %

% \newif\ifbackmatter%
% \newcommand{\backmatter}{\global\backmattertrue}%

% \usepackage[title]{appendix}%

% \@ifpackageloaded{appendix}{%
% %
% \renewenvironment{appendices}{%
%   \@resets@pp
%   \if@dotoc@pp
%     \if@dopage@pp              % both page and toc
%       \if@chapter@pp           % chapters
%         \clear@ppage
%       \fi
%       \appendixpage
%     \else                      % toc only
%        \if@chapter@pp          % chapters
%          \clear@ppage
%        \fi
%       \addappheadtotoc
%     \fi
%   \else
%     \if@dopage@pp              % page only
%       \appendixpage
%     \fi
%   \fi
%   \if@chapter@pp
%     \if@dotitletoc@pp \@redotocentry@pp{chapter} \fi
%   \else
%     \if@dotitletoc@pp \@redotocentry@pp{section} \fi
%     \if@dohead@pp
%       \def\sectionmark##1{%
%         \if@twoside
%           \markboth{\@formatsecmark@pp{##1}}{}
%         \else
%           \markright{\@formatsecmark@pp{##1}}{}
%         \fi}
%     \fi
%     \if@dotitle@pp
%       \def\sectionname{\appendixname}
%       \def\@seccntformat##1{\@ifundefined{##1name}{}{\csname ##1name\endcsname\ }%
%         \csname the##1\endcsname\quad}
%     \fi
%   \fi
% }{%
%   \@ppsaveapp\@pprestoresec}
% %%
% \AtBeginDocument{%
% %
% \let\oldappendices\appendices%
% \let\oldendappendices\endappendices%
% %%
% \renewenvironment{appendices}{%
% \setcounter{figure}{0}%
% \setcounter{table}{0}%
% \setcounter{equation}{0}%
% %%
% \begin{oldappendices}%
%   \gdef\thefigure{\@Alph\c@section\arabic{figure}}%
%   \gdef\thetable{\@Alph\c@section\arabic{table}}%
%   \gdef\theequation{\@Alph\c@section\arabic{equation}}%
% }{\end{oldappendices}}
% }
% %%
% }{}            


% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%% Article History  %%%%%%%%%%%%%%%%%%%%
% %
% \def\@history{}
% \def\printhistory{{\par\addvspace{8pt}%
% \historyfont\noindent%
% \ifx\@history\empty\gdef\@history{Received xx xxx xxxx}\fi\@history\par}}%
% %
% %%%%%%%%%%%%%%%%%%%%%%% Footnotes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% %
% \renewcommand\@makefntext[1]{%
%     \hskip8pt{\smash{\@makefnmark}}#1}
% %
% \RequirePackage{hyperref}%
% %%\RequirePackage{hypcap}%
% \gdef\breakurldefns{%
% \if@pdflatex\else%
%   \RequirePackage[hyphenbreaks]{breakurl}%
% %  \let\href\burlalt%
% \fi}%
% \breakurldefns%
% %    \bgroup
% %      \catcode`\&=12\relax
% %      \hyper@normalise\burl@addtocharlistbefore{%}
% %      \hyper@normalise\burl@addtocharlistafter{:/.?#&_,;!=+~}%% for extra breaks in url
% %    \egroup
% %    \burl@defifstructure
% %
% \hypersetup{%
%         colorlinks,
%         breaklinks=true,
%         plainpages=false,%
%         citecolor=blue,
%         linkcolor=blue,
%         urlcolor=blue,
%         bookmarksopen=true,%
%         bookmarksnumbered=false,%
%         bookmarksdepth=5%
% }
% %
% \AtBeginDocument{\renewcommand\UrlFont{\rmfamily}}%
% %
% \AtBeginDocument{%
% \@ifpackageloaded{natbib}{%
%   \renewcommand\bibsection{%
%    \section*{\refname}%
%   }%
% }{}%
% }%
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% \pagestyle{headings}%
% \pagenumbering{arabic}%
% \sloppy%
% \frenchspacing%
% \flushbottom%

% %%% special parameters for TeX
% \adjdemerits=100
% \linepenalty=100
% %
% %%%%%%%%%%%%%%% Biography
% %
% \RequirePackage{wrapfig}%
% %
% %
% %  \begin{wrapfigure}[12]{r}[34pt]{5cm} <figure> \end{wrapfigure}
% %                     --  -  ----  ---
% %  [number of narrow lines] {placement} [overhang] {width of figure}
% \newcount\wraplines%
% %%\wraplines=5%
% %
% \newbox\@authorfigbox%
% \newskip\@authorfigboxdim%
% %
% \newskip\biofigadjskip%
% \biofigadjskip=0pt%
% %
% \def\authbiotextfont{\reset@font\fontsize{8bp}{9.5bp}\selectfont}%
% %
% \newenvironment{biography}[2]{\par\addvspace{11.5pt plus3.375pt minus1.6875pt}%\lineno@off%
% \def\author##1{{\bfseries##1}}%
% \if!#1!\def\@authorfig{}\else\def\@authorfig{{#1}}\fi%
% \setbox\@authorfigbox=\hbox{#1}%
% \@authorfigboxdim=\wd\@authorfigbox%
% \if@iicol\advance\@authorfigboxdim by -10pt\else\advance\@authorfigboxdim by -2pt\fi%
% \wraplines=9\fboxrule=1pt\fboxsep=6pt%
% \noindent{%
% \ifx\@authorfig\@empty\else\unskip%
% \begin{wrapfigure}[\wraplines]{l}[0pt]{\@authorfigboxdim}%{38.25mm}%
% \vskip-19pt\addvspace{\biofigadjskip}%
% \@authorfig%
% \end{wrapfigure}%
% \fi%
% {\authbiotextfont#2\par}%
% \par%
% }}{\par\addvspace{10.5pt plus3.375pt minus1.6875pt}}
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Theorem %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% %
% \usepackage{amsthm}
% \usepackage{fix-cm}

% \@ifpackageloaded{amsthm}{%
% %
% %\let\proof\relax%
% %\let\endproof\relax%

% \def\@begintheorem#1#2[#3]{%
%   \deferred@thm@head{\the\thm@headfont \thm@indent
%     \@ifempty{#1}{\let\thmname\@gobble}{\let\thmname\@iden}%
%     \@ifempty{#2}{\let\thmnumber\@gobble}{\let\thmnumber\@iden}%
%     \@ifempty{#3}{\let\thmnote\@gobble}{\let\thmnote\@iden}%
%     \thm@swap\swappedhead\thmhead{#1}{#2}{#3}%
%     \the\thm@headpunct
%     \thmheadnl % possibly a newline.
%     \hskip\thm@headsep
%   }%
%   \ignorespaces
% }

% \def\@endtheorem{\endtrivlist\@endpefalse}


% \AtBeginDocument{%
% %
% \DeclareRobustCommand{\S}{\ifmmode\mathsection\else\textsection\fi}

% \DeclareSymbolFont{AMSa}{U}{msa}{m}{n}%
% \DeclareMathSymbol{\opensquare}{\mathord}{AMSa}{"03}%
% \def\qedsymbol{\ensuremath{\opensquare}}%
% %
% \newenvironment{spiproof}[1][\proofname]{\par\removelastskip%\vspace*{2pt}%
%   \pushQED{\qed}%
%   \small\normalfont \topsep7.5\p@\@plus7.5\p@\relax%
%   \trivlist%
%   \item[\hskip\labelsep%
%         \itshape%
%     #1\@addpunct{}]\ignorespaces%
% }{%
%   \popQED\endtrivlist\@endpefalse%
% }%
% %
% \let\proof\spiproof\let\endproof\endspiproof% 
% %
% }%
% %
% \def\thm@space@setup{%
% \thm@preskip=12pt%
% \thm@postskip=12pt}
% %
% %%%%%%%%%%%%%%%%%% StyleOne
% %
% \newtheoremstyle{thmstyleone}% Numbered
% {18pt plus2pt minus1pt}% Space above
% {18pt plus2pt minus1pt}% Space below
% {\small\itshape}% Body font
% {0pt}% Indent amount
% {\small\bfseries}% Theorem head font
% {}% Punctuation after theorem head
% {.5em}% Space after theorem headi
% {\thmname{#1}\thmnumber{\@ifnotempty{#1}{ }\@upn{#2}}%
%   \thmnote{ {\the\thm@notefont(#3)}}}% Theorem head spec (can be left empty, meaning `normal')
% %
% \newtheoremstyle{thmstyletwo}% Numbered
% {18pt plus2pt minus1pt}% Space above
% {18pt plus2pt minus1pt}% Space below
% {\small\normalfont}% Body font
% {0pt}% Indent amount
% {\small\itshape}% Theorem head font
% {}% Punctuation after theorem head
% {.5em}% Space after theorem headi
% {\thmname{#1}\thmnumber{\@ifnotempty{#1}{ }{#2}}%
%   \thmnote{ {\the\thm@notefont(#3)}}}% Theorem head spec (can be left empty, meaning `normal')
% %
% \newtheoremstyle{thmstylethree}% Definition
% {18pt plus2pt minus1pt}% Space above
% {18pt plus2pt minus1pt}% Space below
% {\small\normalfont}% Body font
% {0pt}% Indent amount
% {\small\bfseries}% Theorem head font
% {}% Punctuation after theorem head
% {.5em}% Space after theorem headi
% {\thmname{#1}\thmnumber{\@ifnotempty{#1}{ }\@upn{#2}}%
%   \thmnote{ {\the\thm@notefont(#3)}}}% Theorem head spec (can be left empty, meaning `normal')
% %
% \newtheoremstyle{thmstylefour}% Proof
% {18pt plus2pt minus1pt}% Space above
% {18pt plus2pt minus1pt}% Space below
% {\small\normalfont}% Body font
% {0pt}% Indent amount
% {\small\itshape}% Theorem head font
% {}% Punctuation after theorem head
% {.5em}% Space after theorem headi
% {\global\proofthmtrue\thmname{#1} \thmnote{#3}}% Theorem head spec (can be left empty, meaning `normal')
% %
% }{}

% %% Macros for bibliographystyles %%

% % \def\bibcommenthead{\if@bibcomment\begingroup\parindent=0pt\parskip=0pt%
% % \removelastskip\vskip13pt\nointerlineskip%
% % 
% % \vbox{\bibfont If you are submitting to one of the Nature Research journals, using the eJP 
% %  submission system, please include the references within the manuscript file itself. You may 
% %  do this by copying the reference list from your .bbl file, and pasting it into the bibliography
% %  environment of the main manuscript .tex file.}\par%
% % \removelastskip\nobreak\vskip13pt\nobreak%
% % \endgroup\fi}%

% \def\bibcommenthead{}%

% \if@Spr@basic@refstyle%
%   \if@Numbered@refstyle%
%     \RequirePackage[backend=biber,style=numeric,sorting=none]{biblatex}%
%     \gdef\NumBib{YES}%
%   \else%
%     \RequirePackage[backend=biber,style=authoryear]{biblatex}%
%     \gdef\NumBib{NO}%
%     \setcitestyle{aysep={}}%
%   \fi%
%   \setlength{\bibsep}{1em}%
%   \def\bibfont{\reset@font\fontfamily{\rmdefault}\normalsize\selectfont}%
% \fi%

% \if@Mathphys@numrefstyle%
%   \RequirePackage[backend=biber,style=numeric,sorting=none]{biblatex}%
%   \gdef\NumBib{YES}%
%   % \setlength{\bibsep}{1em}%
%   \def\bibfont{\reset@font\fontfamily{\rmdefault}\normalsize\selectfont}%
% \else%
%   \if@Mathphys@ayrefstyle%
%     \RequirePackage[backend=biber,style=authoryear]{biblatex}%
%     \gdef\NumBib{NO}%
%     \setcitestyle{aysep={}}%
%     \setlength{\bibsep}{1em}%
%     \def\bibfont{\reset@font\fontfamily{\rmdefault}\normalsize\selectfont}%
%   \fi%
% \fi%

% \if@APS@refstyle%
%   \RequirePackage[backend=biber,style=numeric,sorting=none]{biblatex}%
%   \gdef\NumBib{YES}%
%   \setlength{\bibsep}{1em}%
%   \def\bibfont{\reset@font\fontfamily{\rmdefault}\normalsize\selectfont}%
% \fi%

% \if@Vancouver@numrefstyle%
%   \RequirePackage[backend=biber,style=numeric,sorting=none]{biblatex}%
%   \gdef\NumBib{YES}%
%   \setlength{\bibsep}{1em}%
%   \def\bibfont{\reset@font\fontfamily{\rmdefault}\normalsize\selectfont}%
% \else%
%   \if@Vancouver@ayrefstyle%
%     \RequirePackage[backend=biber,style=authoryear]{biblatex}%
%     \gdef\NumBib{NO}%
%     \setcitestyle{aysep={}}%
%     \setlength{\bibsep}{1em}%
%     \def\bibfont{\reset@font\fontfamily{\rmdefault}\normalsize\selectfont}%
%   \fi%
% \fi%

% \if@APA@refstyle%
%   \if@Numbered@refstyle%
%     \RequirePackage[backend=biber,style=apa]{biblatex}%
%     \gdef\NumBib{YES}%
%   \else%
%     \RequirePackage[backend=biber,style=apa]{biblatex}%
%     \gdef\NumBib{NO}%
%   \fi%
%   \def\refdoi#1{\urlstyle{rm}\url{#1}}%
%   \renewcommand{\doiprefix}{}%
%   \AtBeginDocument{%
%     \renewcommand{\BPBI}{.}% Period between initials
%   }%
%   \setlength{\bibsep}{1em}%
%   \def\bibfont{\reset@font\fontfamily{\rmdefault}\normalsize\selectfont}%
% \fi%

% \if@Chicago@refstyle%
%   \if@Numbered@refstyle%
%     \RequirePackage[backend=biber,style=numeric,sorting=none]{biblatex}%
%     \gdef\NumBib{YES}%
%   \else%
%     \RequirePackage[backend=biber,style=authoryear]{biblatex}%
%     \gdef\NumBib{NO}%
%     \setcitestyle{aysep={}}%
%   \fi%
%   \hypersetup{urlcolor=black,colorlinks=false,pdfborder={0 0 0}}%
%   \urlstyle{same}%
%   \setlength{\bibsep}{1em}%
%   \def\bibfont{\reset@font\fontfamily{\rmdefault}\normalsize\selectfont}%
% \fi%

% \if@Standard@Nature@refstyle%
%   \RequirePackage[backend=biber,style=numeric,sorting=none]{biblatex}%
%   \gdef\NumBib{YES}%
%   \setlength{\bibsep}{1em}%
%   \def\bibfont{\reset@font\fontfamily{\rmdefault}\normalsize\selectfont}%
% \fi%


% \endinput

